Braided multitwists

We provide a characterization for multitwists satisfying the braid relation in the mapping class group of an orientable surface.

==> contenido/otrosautores.tex <==
El resultado que presentamos en este artículo forma parte del  ecosistema de teoremas que establecen un diccionario entre propiedades topológicas y propiedades algebraicas del $\mcg(S)$. En esta sección resumimos algunos resultados colindantes al Teorema \ref{thm1}.

En general, distintos autores han tenido interés en establecer condiciones para que dos multigiros $\tau_A$ y $\tau_B$  generan un grupo libre. Pero esto solo se hace de manera efectiva para multigiros positivos. En el caso de Margalit, es ligeramente diferente (leer abajo).

Las técnicas utilizadas son esecialmente tres:
\begin{itemize}
    \item Utilizar la construcción de Thurston para determinar cuando dos multigiros generan un pseudo-anosov. 
    \item Utilizar las fórmulas del número de intersección para multigiros del mismo signo más el lema del ping-pong.
    \item Utilizar la fórmula del número de intersección algebraico. 
\end{itemize}

Por tanto, nuestra aproximación parece ser diferente. No intenta hacer algo tan ambicioso como caracterizar cuando generan un grupo libre (nos contentamos con encontrar la relación de trenza), pero a cambio podemos usar multigiros con exponentes arbitrarios. Además, uso una fórmula de Ivanov que no parece estar siendo usada en ningún sitio. Ni siquiera la usa el mismo Ivanov porque está escondida en su demostración.


\subsection*{John McCarthy}
Los primeros resultados caracterizando topológicamente giros de dehn en términos de propiedades algebraicas los encontré en el artículo \cite{mccarthy_automorphisms_1986} de McCarthy. En el Lema 4.3 recoge resultados que probablemente fuesen ya conocidos: dos giros de dehn conmutan si y solo si sus curvas son disjuntas; dos giros de dehn satisfacen la relación de trenzas si y solo si tienen el mismo exponente $1$ o $-1$ y las curas se intersecan una vez. 

\subsection*{Hamidi-Tehrani}
En \cite{hamidi-tehrani_groups_2002} Hamidi-Tehrani incluye dos resultados principales:

Por un lado, da algunas condiciones bajo las cuales los dos multigiros generan un grupo libre (Leininger mejora significativamente este resultado).

Por otro lado, da condiciones bajo las cuáles el conjunto de  giros de dehn $\{\delta_{a_1},\dots, \delta_{a_h} \}$ generan un grupo libre $\mathbb{F}_h$. Sea $m>0$ el mínimo número de intersección entre las curvas y $M$ el máximo, la condición es $M\leq m^2/6$. 

Este último resultado parece fuerte, pero nótese que no nos va a decir absolutamente nada para el caso en que tenemos multigiros. Porque para que el resultado sea interesante necesita que la intersección mínima sea mayor que cero. 

Su demostración esencialmente juega con el número de intersección usando la fórmula para multigiros positivos, y el lema del ping-pong.

\subsection*{Leininger}

En \cite{leininger_groups_2004} Leininger da una caracterización completa de cuándo dos multigiros positivos generan un grupo libre. Aquí se necesita fuertemente que los multigiros sean positivos (o del mismo signo, da igual). 

Su prueba es esencialmente llevar hasta el final la construcción de Thurston en \cite{thurston_geometry_1988} sobre cuándo dos multigiros generan un elemento pseudo-Anosov. Luego, da una caracterización de esa situación en términos de grafos que describen la intersección entre las curvas. 


\subsection*{Dan Margalit}
En \cite{margalit_lantern_2002} Margalit utiliza la fórmula del número de intersección algebraico y la fórmula del número de intersección para multigiros positivos.

Su resultado describe cuando dos giros de dehn  forman una linterna o una 2-cadena. Para ambos resultados se remite únicamente al caso en que tiene dos giros de dehn en uno de los lados de la igualdad: \[\delta_a^k \delta_b^j = M.\]Este resultado contrasta con el nuestro, que lidia con una cantidad arbitraria de giros de dehn. No tengo del todo claro que haya una forma de pasar de su resultado al de este artículo. 

\subsection*{Blazej Szepietowski}
El Corolario \ref{cor1} se puede interpretar como una caracterización de ciertos embebimientos del grupo de tres trenzas $B_3$ en $\mcg(S)$.  Concretamente, se caracterizan todos los embebimientos $B_3 \hookrightarrow \mcg(S)$ que envían un generador estándar de $B_3$ en un multigiro. 

Este tipo de resultados ha sido bien estudiado. Aunque uno querría generalizar este resultado para caracterizar todos los embebimientos de $B_3$ en $\mcg(S)$, Blazej Szepietowski nos da las malas noticias. En el artículo \cite{szepietowski_embedding_2010} Szepietowski construye un embebimiento del grupo de trenzas en $\mcg(S)$ de manera que la imagen de un generador estándar es una raíz no trivial de un multigiro. Esto nos frena los pies en seco. 

\subsection*{Hay más autores}

Seguramente haya muchos autores que estoy dejando por fuera. 


==> contenido/personal.tex <==

Toda esta idea de utilizar homología parece sacada de la manga. No, señor, eso solo es así porque a posteriori me he quedado con lo mínimo necesario para llevar acabo el argumento de la prueba. Pero en realidad todo encaja de forma muy natural. En esta sección intentaré replicar lo que pasó por mi mente en ese momento.

Al principio lo estuve intentando únicamente con dos curvas en $A$ y en $B$. Lo primero que uno observa es la correspondencia que hicimos al principio de la Sección \ref{sec:almeollo}, esto es, que tenemos una correspondencia $\tau_A\tau_B\cdot a_i =b_i$, que de paso fuerza que los exponentes sean iguales. Después, intenté conseguir contradicciones para varias configuraciones de curvas utilizando el número de intersección y la observación de que $i(a_i,b_i) = i(a_i, \tau_A\tau_B\cdot a_i) = i(a_i,\tau_B\cdot a_i)$.
Llegados a ese punto me estanqué un poco porque todas las fórmulas que hay asumen que el multigiro es positivo. Allí fue cuando me remití (guiado por el Farb-Margalit) a la estimación de Ivanov. Como la estimación no me fue demasiado útil, salvo para descartar algunos casos, entonces me adentré en la demostración. Fue allí cuando descubrí la fórmula perdida de Ivanov de la Subsección \ref{subsec:formulaivanov}. 

Una vez llegados allí, me di cuenta que la fórmula me daba la clasificación de configuraciones de curvas que esbozo en la Subsección \ref{subsec:clasificacion}. Aquí hubo de nuevo un buen parón, no sabía cómo continuar y descartar las configuraciones que no eran las elementales. Incluso me llegué a preguntar si no habría alguna otra configuración de multigiros que también satisfaciera la relación de trenzas. Fue hacer varios ejemplos (para probar o desmentir esa teoría) lo que me dio cierta intuición de lo que estaba pasando. 

Entonces se me ocurrió ver cómo eran las intersecciones de las curvas localmente y me di cuenta que salvo intersecciones pequeñas (que quizás manejaría a parte), podía asegurarme de que el homeomorfismo $h=(\tau_A\tau_B\tau_A)^2$ iba a fijar todas las curvas y usando el método de Alexander podría demostrar $h\simeq \text{id}$. 

Ahora, yo sabía que en el caso `clásico' $h \not \simeq \text{id}$, sino que $h^2 \simeq \text{id}$. Solo me hacía falta ver de dónde venía que no fuese homotópico a la identidad. Si uno se fijaba solo en las curvas $A\cup B$ (y en el número de intersección), entonces no se veía ninguna incongruencia ¿Entonces podía aplicar el método de Alexander? No! Porque las orientaciones no se fijaban. Se me iluminó la bombilla y ¡Eureka! en las curvas no puedes ver la incongruencia, pero deberías poder verla en la homología. Voy pongo la idea a prueba y funciona... 

Entre que me plantee este problema seriamente y conseguí resolverlo pasaron aproximadamente 11 meses. Así que obviamente hay muchas cosas que estoy pasando por alto, y estoy quizás haciendo demasiado énfasis en lo que sucedió hacia el final de este periodo. Pero, por lo menos, se captura el origen de algunas de las ideas que tuve. Es curioso, no hubo magia, solo una construcción continua, una apisonadora que con el tiempo domesticó al problema. Y, de paso, en el proceso aprendí un montón de cosas sobre train-tracks y pseudo-Anosovs, que no utilicé pero que son interesantes por sí mismas. 


